Importance Sketching of Influence Dynamics in Billion-scale Networks

The blooming availability of traces for social, biological, and communication networks opens up unprecedented opportunities in analyzing diffusion processes in networks. However, the sheer sizes of the nowadays networks raise serious challenges in computational efficiency and scalability. In this paper, we propose a new hyper-graph sketching framework for inflence dynamics in networks. The central of our sketching framework, called SKIS, is an efficient importance sampling algorithm that returns only non-singular reverse cascades in the network. Comparing to previously developed sketches like RIS and SKIM, our sketch significantly enhances estimation quality while substantially reducing processing time and memory-footprint. Further, we present general strategies of using SKIS to enhance existing algorithms for influence estimation and influence maximization which are motivated by practical applications like viral marketing. Using SKIS, we design high-quality influence oracle for seed sets with average estimation error up to 10x times smaller than those using RIS and 6x times smaller than SKIM. In addition, our influence maximization using SKIS substantially improves the quality of solutions for greedy algorithms. It achieves up to 10x times speed-up and 4x memory reduction for the fastest RIS-based DSSA algorithm, while maintaining the same theoretical guarantees.

==> body/hardness.tex <==
%\subsection{Properties}

%The 
%- Only difference from Influence by a fixed factor $|S|$ $\leftrightarrow$ interchangeable. 

%- Comparing nodes' influence might lead to wrong perception about nodes importance. For example, comparing "raw" influences nodes $a$ \& $b$ have influence 1.2 \& 1.11 respectively, which suggest $a$ \& $b$ have roughly same influence. Indeed, $a$ is much more influenced than $b$, ($a$ has external value 0.2) \& $b$ has external influence 0.11.
%The first property of outward influence compared to the normal definition of influence is the better distinction of nodes' importance in the network while comparing the influence may lead to wrong perception. Take an example in Fig.~\ref{fig:example}, nodes $a$ and $b$ have influences of $1+p+p^2$ and $1+2\cdot p$, respectively, which are roughly the same, $\frac{1+p+p^2}{1+2\cdot p} \approx 1$. In fact, $b$ is intuitively much more influential than $a$ since it directly connects to both $a$ and $c$. Indeed, the outward influences of the two nodes captures accurately that intuition of node $b$ is almost twice as influential as $a$, $\frac{\I_E(b)}{\I_E(a)} \approx 2$.


%\todo{Redraw the figures and make a table to compare influence vs. outward influence as the Figure 1 in the Wei Chen's paper \url{https://arxiv.org/pdf/1602.03780v4.pdf} }

%\begin{figure}[h!] \centering
%	\includegraphics[width=1.7in]{figures/example}
%	\caption{note figure.}
%	\label{fig:example}
%\end{figure}

%\setlength\tabcolsep{4pt}
%\def\arraystretch{1.1}
%\begin{figure}[t]
%	\begin{minipage}[t]{0.26\textwidth} \centering
%		\vspace{-0.8in}
%		\begin{tabular}{lll}
%			\toprule
%			$S$ & $\I(S)$ & $\I_E(S)$ \\
%			\midrule
%			$\{a\}$ & $1+p + p^2$ & $p+p^2$ \\
%			$\{b\}$ & $1 + p + p = 1+ 2\cdot p$ & $2\cdot p$ \\
%			$\{a,b\}$ & $2 + p$ & $p$ \\
%			$\{a,d\}$ & $2 + 2\cdot p + p^2$ & $2\cdot p + p^2$\\
%			\bottomrule
%		\end{tabular}
%		%		\caption{Compute $\I(S)$ and $\I_E(S)$}
%		%		\label{tab:cpu_gpu}
%	\end{minipage}%
%	\begin{minipage}[t]{0.3\textwidth} \centering
%		\includegraphics[width=0.8in]{figures/example}
%		\vspace{-4in}
%		%			\caption{Example Graph}
%		%			\label{fig:example}
%	\end{minipage}
%	\vspace{-0.05in}
%	\caption{Example with 5 nodes (edge probability $p$)}
%	\vspace{-0.15in}
%	\label{fig:example}
%\end{figure}

\subsection{Outward Influence Properties}
\textbf{Better Influence Discrimination.} As pointed out in the introduction, outward influence is better than influence spread when comparing the relative influence among the nodes. 
For example, nodes $a$ and $b$ in Fig.~\ref{fig:example} have influence spreads of $1+p+p^2$ and $1+2\cdot p$, respectively. Thus one can mistakenly think $a$ is as influential as $b$. In fact, $b$ is intuitively much more influential than $a$ since it directly connects to both $a$ and $c$. The outward influences of the two nodes accurately reflect that $b$ is almost twice as influential as $a$, since $\frac{\I_E(b)}{\I_E(a)} \approx 2$ when $p$ approaches $0$.
Thus outward influence can be adopted as a better nodes' importance measure. 

\textbf{Non-monotonicity.} Outward influence as a function of seed set $S$ is not monotone. This is different from the influence spread due to the exclusion of self-influence.

Let revisit the example in Figure~\ref{fig:example}. There are 3 nodes and 2 edges with the same weights of $p=0.1$ in the graph. Consider the set having only the node $a$, $\{a\}$ with $\I_E(\{a\}) = 0.11$, if we add $b$ into it to get $\{a,b\}$, the outward influence decreases to $0.1$. However, adding node $c$ instead of $b$, the outward influence increases to $0.19$. Therefore, adding nodes may increase or decrease the outward influence and thus, the function is non-monotone.

\textbf{Submodularity.} Submodularity is a natural property that has been observed and widely applied in many real-world problems, e.g., viral marketing \cite{Kempe03}, sensor placements \cite{Krause08}, diseases outbreak detection \cite{Leskovec07}. Submodularity expresses the diminishing returns behavior of set functions, that adding nodes earlier is always more beneficial than doing that later.

Similar to the traditional influence function, the outward influence is also submodular.
\begin{Lemma}
	\label{lem:submod}
	Given a network $G = (V,E,w)$, the outward influence function $\I_E(S), S \in 2^{|V|},$ is submodular. For any pair of seed sets $S, T$ such that $S \subseteq T \subseteq V$ and $v \in V\backslash T$,
	\begin{align}
		\I_E(S \cup \{v\}) - \I_E(S) \geq \I_E(T \cup \{v\}) - \I_E(T).
	\end{align}
\end{Lemma}
\begin{proof}
%	To prove Lemma~\ref{lem:submod}, we first define the probability space over all the possible \textit{sampled graphs} of the probabilistic graph $\G = (V,E,w)$. Recall that each edge $(u,v) \in E$ is associated with a probability $w(u,v)$ of $u$ successfully influencing $v$ if $u$ gets influenced and $v$ does not. That is equivalent to flipping a coin of bias $w(u,v)$ to specify whether $u$ succeeds. If the coin landed heads for the edge $(u,v)$, we call $(u,v)$ a \textit{live} edge. Since all the influence trials through edges are independent from each other, it does not matter when the coin flips are performed, when $u$ gets influenced or before that point. Therefore, we can flip all the coins at the beginning of the cascade and get a \textit{sampled graph} $g = (V,E')$ where $E' \subseteq E$ contains only the live edges.
%	
%	Hence, we define a probability space $\Omega_\G$ in which a sample point represents a particular sampled graph $g \in \Omega_\G$ where coins are flipped and a set of live edges are determined. Each sampled graph $g \in \Omega_\G$ has a probability of being realized from $\G$, denoted by $\Pr[g \sim \G]$, that depends on the set of live edges in $E'$ of $g$,
%	\begin{align}
%		\Pr[g \sim \G] = \prod_{(u,v) \in E'} w(u,v) \prod_{(u,v) \notin E'} (1-w(u,v))
%	\end{align}
%	
	Recall that on a sampled graph $g \sim \G$, for a set $S \subseteq V$, we denote $\eta_g(S)$ to be the set of nodes, excluding the ones in $S$, that are reachable from $S$ through live edges in $g$. Alternatively, $\eta_g(S)$ is called a sampled outward influence of $S$ on sample $g$ and, consequently, we have,
	\begin{align}
		\I_E(S) = \sum_{g \sim \G} |\eta_g(S)| \Pr[g \sim \G].
		\label{eq:compute_ie}
	\end{align}
	
	Let consider a sampled graph $g \sim \G$, two sets $S, T$ such that $S \subseteq T \subseteq V$ and a node $v \in V \backslash T$. We have three possible cases:
	\begin{itemize}
		\item \textbf{Case $v \in \eta_g(S)$}: then $v \in \eta_g(T)$ since $S \subseteq T$ and $v \notin T$. Thus, we have the following,
		\begin{align}
			\eta_g(S \cup \{v\}) - \eta_g(S) = \eta_g(T \cup \{v\}) - \eta_g(T) = -1. \nonumber
		\end{align}
		\item \textbf{Case $v \notin \eta_g(S)$ but $v \in \eta_g(T)$}: We have that,
		\begin{align}
			\eta_g(S \cup \{v\}) - \eta_g(S) = |\eta_g(\{v\}) \backslash (\eta_g(S) \cup S)| \geq 0
		\end{align}
		while $\eta_g(T \cup \{v\}) - \eta_g(T) = -1$. Thus,
		\begin{align}
			\eta_g(S \cup \{v\}) - \eta_g(S) > \eta_g(T \cup \{v\}) - \eta_g(T).
		\end{align}
		\item \textbf{Case $v \notin \eta_g(T)$}: Since $\forall u \in \eta_g(S) \cup S$, either $u \in \eta_g(T)$ or $u \in T$ or $\eta_g(S) \cup S \subseteq \eta_g(T) \cup T$, we have,
		\begin{align}
			\eta_g(S \cup \{v\}) - \eta_g(S) &= |\eta_g(\{v\}) \backslash (\eta_g(S)\cup S)| \nonumber \\
			& \geq |\eta_g(\{v\}) \backslash (\eta_g(T) \cup T)| \nonumber \\
			& = \eta_g(T \cup \{v\}) - \eta_g(T).
		\end{align}
	\end{itemize}
	In all three cases, we have,
	\begin{align}
		\label{eq:sub_g}
		\eta_g(S \cup \{v\}) - \eta_g(S) \geq \eta_g(T \cup \{v\}) - \eta_g(T).
	\end{align}
	Applying Eq.~\ref{eq:sub_g} on all possible $g \sim \G$ and taking the sum over all of these inequalities give
	\begin{align}
		\sum_{g \sim \G}(\eta_g&(S \cup \{v\}) - \eta_g(S)) \Pr[g \sim \G] \nonumber \\
		&\geq \sum_{g \sim \G}(\eta_g(T \cup \{v\}) - \eta_g(T)) \Pr[g \sim \G],
	\end{align}
	or,
	\begin{align}
		\I_E(S \cup \{v\}) - \I_E(S) \geq \I_E(T \cup \{v\}) - \I_E(T).
	\end{align}
	That completes the proof.
\end{proof}

\subsection{Hardness of Computation} 
%-\todo{\#P-completeness}

Our first hardness result is that computing the outward influence of any set of nodes is \#P-hard. This is directly due to the difference by a constant $|S|$ between outward influence and the influence spread of the set $S$. \#P-hardness property of computing influence was previously proved in the work of Chen et al. \cite{Chen10} and if there exists an algorithm for computing outward influence in polynomial time, we can just add $|S|$ into the outward influence and obtain a polynomial time influence computation algorithm.

%-\todo{Exponentially small vs. lower-bounded by $|S|$ as for node influence}

However, differ from influence spread being at least $|S| \geq 1$, the outward influence of any set $S$ can be arbitrarily small. Take an example in Figure~\ref{fig:example}, node $a$ has influence of $\I(\{a\}) = 1+p+p^2 \geq 1$ for any value of $p$. However, $a$'s outward influence $\I_E(\{a\}) = p + p^2$ can be exponentially small as $p$ approaches $0$. This creates a huge challenge in estimating the measure with high accuracy.

In particular, we are desirably interested in having an $(\epsilon,\delta)$-approximation in the form,
\begin{align}
	\Pr[ (1 - \epsilon) \I_E(S) \leq  \hat \I_E(S) \leq  (1 +  \epsilon) \I_E(S)] \geq 1-\delta
\end{align}
where $\hat \I_E(S)$ is an estimate of $\I_E(S)$. The smaller the values of $\epsilon,\delta$, the better $\hat \I_E(S)$.

%-\todo{ Monte-Carlo Simulation requires exponential number of samples}

To estimate $\I(S)$, one can use Monte-Carlo method to simulate many influence propagations and take the average results of the outward influences as an estimation. Since the influence of a seed set $S$ is at least $|S|\geq 1$, we only need a polynomial times number of samples to have an $(\epsilon, \delta)$ estimation of $\I(S)$ \cite{Dagum00}. In contrast, the number of samples necessary to obtain an ($\epsilon$, $\delta$)-approximation for $\I_E(S)$ is at least $c\frac{1}{\epsilon^{2}}\log{\frac{1}{\delta}}\frac{n}{\I_E(S)}$, where $c$ is some constant. As $\I_E(S)$ can be exponentially small, the number of samples for estimating $\I_E(S)$ can be exponentially large. Note that we cannot obtain an $(\epsilon,\delta)$-approximation of $\I_E(S)$ through $\I(S)$ since the additive $|S|$ difference does not preserve the multiplicative $1\pm\epsilon$. Even worse, the relationship between their approximation guarantees is unknown.

For the same reason, the recent advances in influence estimation in \cite{Borgs14, Lucier15} cannot be adapted to obtain polynomial-time $(\epsilon, \delta)$ estimation for outward influence. We shall address this challenging task  in the next section.

%Given a set of seed nodes $S \subseteq V$, let $I_S$ be the random variable that indicates the number of influenced nodes by $S$ (according to the IC model) and $X_S = I_S - |S|$ denotes the number of influenced ndoes excluding the nodes in $S$. We aim to compute ($\epsilon$, $\delta$)-approximations of:
%
%To estimate $\I(S)$, one can use Monte-Carlo method to simulate the influence propagation and take the average results as estimations. The number of simulations/samples necessary to give an ($\epsilon$, $\delta$)-approximations for $I(S)$ is at least $c\frac{1}{\epsilon^{2}}\log{\frac{1}{\delta}}\frac{n}{I(S)}$
%
%\[\I(S) = E[I_S] \text{, termed the influence of $S$}\]
%
%and
%\[\I_E(S) = E[X_S] = E[I_S - |S|] = \I(S) - |S|, \] termed the external influence of $|S|$
%
%
%
%\todo{Advanced Influence Estimation (KDD'15) cannot be Applied}
%
%A recent approach in KDD'15 improves the running time and reduce the number of observed influences to $O(nlog^5n)$ \cite{Lucier15}. We show in the appendix that, indeed, only $O(n)$ observed influences are sufficient. Thus, we improve the running time by a factor $O(log^5n)$.
%
%To estimate $I_E(S)$, all of the above methods do not work. The reason is that the number of required samples $c\frac{1}{\epsilon^{2}}\log{\frac{1}{\delta}}\frac{n}{I_E(S)}$ can be exponentially large as $I_E(S)$ can be as small as $e$. Because of this, design an \FPRAS{} for $I_E(S)$ is an nontrivial task.

==> body/issa.tex <==
\begin{algorithm}[!ht] \small
	\caption{\ISSA{} Algorithm}
	\label{alg:dpima}
	\KwIn{Graph $G$, $k$, desired approximation ratio $0 \leq \rho$ and probability guarantee $\delta$}
	\KwOut{ $\hat S_k$ and its approximation guarantee $\rho_t$}
	$\epsilon = (1-\frac{1}{e}) - \rho$; 
	%	\If{$\rho > 1-\frac{1}{e}$}{$\epsilon = 0.1$;}
	$\epsilon_0 = \max\{\epsilon, 0.1\}$; \\
	$N_{\max} = \min\{ \Upsilon\left(\epsilon, \frac{\delta}{6}/{n\choose k}\right)\frac{n}{k}, n^2 \}$; \\
	$t_{\max} = \lceil \log_2 (N_{\max}/ \Upsilon(\epsilon_0, \frac{\delta}{3})) \rceil$; $t = 0$;\\
	$\Lambda = \Upsilon(\epsilon_0, \frac{\delta}{3 t_{\max}}); \Lambda_1 = 1+(1+\epsilon_0) \Upsilon(\epsilon_0, \frac{\delta}{3 t_{\max}})$; \\
	\Repeat{$|\R_t|\geq N_{\max}$}{
		$t = t + 1$; \\
		$\R_t = \{ R_1, \dots, R_{\Lambda2^{t-1}} \}$; $\R^{c}_t = \{ R_{\Lambda2^{t-1}+1}, \dots, R_{\Lambda 2^t} \}$; \\
		$<\hat S_k, \hat \I^{(c)}_t(\hat S_k), \sigma> \leftarrow \textsf{Greedy}(\R_t, k)$;\\
		\If{$\I_t^{(c)}(\hat S_k) \cdot |\R^c_t|/n \geq \Lambda_1
			$}{
			%			$\I^{c}_t(\hat S_k) \leftarrow \Cov_{\R^{c}_t}(\hat S_{k})\cdot n/|\R^{c}_t|$;\\
			$\epsilon_1 \leftarrow \hat \I_t(\hat S_k)/{\hat \I}^{(c)}_t(\hat S_k) - 1$;\\
			$\epsilon_2 \leftarrow \epsilon_0 \sqrt{\frac{n(1+\epsilon_0)}{2^{t-1} {\hat \I}^{(c)}_t (\hat S_k)}}$; $\epsilon_3 \leftarrow \epsilon_0 \sqrt{\frac{n(1+\epsilon_0)\rho}{(1+\frac{\epsilon_0}{3})2^{t-1} {\hat \I}^{(c)}_t (\hat S_k)}}$;\\		
			$\rho_t = \sigma(1-\epsilon_3)-(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2)\rho$;\\
			\If{$\rho_t \geq \rho$} {\textbf{return} $<\hat S_k, \rho_t>$; }
			%			\If{$(\epsilon \leq 0) \emph{\textbf{ and }} (|\epsilon_1| + \epsilon_2 + \epsilon_3 < \epsilon_{small })$}{\textbf{return} $<\hat S_k, \rho_t>$ }
		}
	}
	\textbf{return} $<\hat S_k, \max \{\rho_t ,1-1/e-|\epsilon|\}>$;
\end{algorithm}

\subsection{ISSA Approximation Algorithm}

We combine the new \ROS{} sketch and runtime approximation bound with the recent Stop-and-Stare framework \cite{Nguyen163} to propose \ISSA{}. The combined method can provide a runtime approximation guarantee beyond $1-1/e$.

\subsubsection{Algorithm Description}
The detailed description of \ISSA{} is presented in Alg.~\ref{alg:dpima}. In addition to the graph $\G$, number of selected seeds $k$, the algorithm takes in a value $\rho$ which is the desired approximation ratio that a user would like to obtain. Traditionally, $\rho = 1-1/e-\epsilon$ for some $\epsilon$, however, the runtime approximation bound gives \ISSA{} the opportunities to provide better guarantees on a particular execution of \ISSA{}.

Initially, it computes the value of $\epsilon$ (Line~1) which is the gap from the desired $\rho$ to $1-1/e$ and $\epsilon_0$. $\epsilon$ is used to set the maximum necessary \ROS{} samples $N_{\max}$ (Line~2) and $\epsilon_0$ decides the initial \ROS{} samples generated $\Lambda$ (Line~4). $t_{\max}$ is the maximum number of iterations in the main loop (Line~5-17) and computed by the logarithm based 2 of $\frac{N_{\max}}{\Lambda}$. The precomputed $\Lambda_1$ (Line~4) serves in the first stopping condition (Line~10) which provides a certain bound on the solution quality. The main body of \ISSA{} is a loop in which two sets of \ROS{} samples are used: $\R_t$ with $\Lambda \cdot 2^{t-1}$ \ROS{} (Line~7) for finding the candidate seed set $\hat S_k$ by the \textsf{Greedy} with runtime approximation bound (Line~9) and $\R_t^{(c)}$ with the same number of samples for reestimating the influence of $\hat S_k$.

The error bound in iteration $t$ is calculated in Lines~11-14 and if it meets the required approximation ratio (Lines~15-16), then \ISSA{} terminates and returns $\hat S_k$. Checking the approximation guarantee is only one of three stopping conditions. Another condition is taken from \cite{Tang15} which bounds the maximum number of samples needed to provide the bound $\rho$ in cases where $\rho \leq 1-1/e-\epsilon$ for some $0 < \epsilon < 1$. This plays as a guarding condition to stop the algorithm when $\rho > 1-1/e$ and it is not possible to achieve that desired approximation guarantee. In that case, \ISSA{} returns a solution $\hat S_k$ with guaranteed ratio of $\max\{1-1/e-|\epsilon|,\rho_t\}$.

\subsubsection{Optimality Guarantees Analysis}
We prove that when $\rho < 1-1/e$, \ISSA{} returns a seed set $\hat S_k$ of size $k$ that is at least $\rho$-optimal with probability at least $1-\delta$. Furthermore, in that case, \ISSA{} requires at most the type-2 optimal number of \ROS{} samples. The type-2 \cite{Nguyen163} is defined as the minimum samples to guarantee an $(1-1/e-\epsilon)$-optimal solution where $\epsilon = (1-1/e)-\rho$ with probability at least $1-2\delta$.

In the other cases of $\rho \geq 1-1/e$, \ISSA{} has a chance return a solution $\hat S_k$ meeting the desired $\rho$ when the stopping condition $\rho_t \geq \rho$ is met. That depends mostly on the runtime approximation bound. In cases where $\rho_t \geq \rho$ can not be satisfied, the cap $N_{max}$ on the number of \ROS{} samples will terminate the algorithm and provides the best-effort guarantee of $\max\{ \rho_t, 1-1/e-|\epsilon| \}$.

\textbf{Approximation Guarantee.}
For clarity, we present most of the proofs in the appendix.

%In our proofs, we make good uses of the following results on probability bounds. 

Recall that \ISSA{} stops when either 1) the number of samples exceeds the cap, i.e., $|\R_t| \geq N_{\max}$ or 2) $\rho_t \geq \rho$ for some $t \geq 1$. In the first case,  $N_{\max}$ were chosen to guarantee that 
$\hat S_k$ will be a $(1-1/e-\epsilon)$-approximation solution w.h.p.
\begin{Lemma}
	\label{lem:cap}
	Let $B^{(1)}$ be the bad event that 
	%\vspace{-0.05in}
	\[
		B^{(1)} = (|\R_t| \geq N_{\max}) \cap (\I(\hat S_k) < (1-1/e-\epsilon)\emph{\OPT}_k).
	\] where $\epsilon = (1-1/e) - \rho > 0$ since we are considering $\rho < 1-1/e$. We have
	%\vspace{-0.05in}
	\[
	\Pr[B^{(1)}] \leq  \delta/3.
	\]
\end{Lemma}

This results is followed directly from \cite{Tang15} replacing $\delta$ with $\delta/3$. In the second case, the algorithm stops when $\epsilon_t \leq \epsilon$ for some
$1\leq t \leq t_{\max}$. The maximum number of iterations $t_{\max}$ is bounded by $O(\log n)$ as stated below.
\begin{Lemma}
	\label{lem:tmax}
	The number of iterations in \ISSA{} is at most $t_{\max} = O(\log n)$.
\end{Lemma}

For each iteration $t$, we will bound the probabilities of the bad events that lead to inaccurate estimations of  $\I(\hat S_k)$ through $\R^{c}_t$, and $\I(S^*_k)$ through $\R_t$(Lines~12 and~13).

\begin{Lemma}
	\label{lem:bad2}
	For each $1\leq t \leq t_{\max}$, let 
	%\vspace{-0.05in}
	\[
	\hat \epsilon_t \text{ be the unique root of } f(x)=\frac{\delta}{3t_{\max}},
	\]
	%\vspace{-0.15in}
	
	\noindent where $f(x)=\exp{\left(-\frac{N_t \frac{\I(\hat S_k)}{n} x^2 }{2+2/3x}\right)}$, and 
	%\vspace{-0.05in}
	\[
	\epsilon_t^*=
	\epsilon_0 \sqrt{\frac{n}{(1+\epsilon_0/3)2^{t-1} \emph{\OPT}_k}}.
	\]
	%\vspace{-0.15in}
	
	\noindent Consider the following bad events
	%\vspace{-0.05in}
	\begin{align*}
	%B_t^{(2)} &=  \left(\I^{c}_t(\hat S_k) \geq (1 + \epsilon)\I(\hat S_k)	\right) \text{given } \left(\Cov_{\R^{c}_t}(\hat S_k) \geq \Lambda_1\right)\\
	B_t^{(2)} &= \left(
	\hat \I_t^{(c)}(\hat S_k) \geq (1+\hat \epsilon_t)\I(\hat S_k) \right),
	\\
	B_t^{(3)} &= \left(
	\hat \I_t(S^*_k) \leq (1-\epsilon_t^*) \emph{\OPT}_k]
	\right).
	% \\ 
	%B_t^{(4)} &= \left(
	%\hat \I_t^{(c)}(\hat S_k) \geq \I(\hat S_k) + \epsilon^*_t \OPT_k
	% \right).
	\end{align*}
	%\vspace{-0.25in}
	
	\noindent We have 
	%\vspace{-0.05in}
	\[
	\Pr[B_t^{(2)}],  \Pr[B_t^{(3)}] \leq \frac{\delta}{3t_{\max}}.
	\]
	%\vspace{-0.2in}
\end{Lemma}
%\begin{proof} One can verify that $f(x)$ is a strictly decreasing function for $x>0$. Moreover, $f(0)=1$ and $\lim_{x\rightarrow \infty} f(x) = 0$. Thus, the equation $f(x)=\frac{\delta}{3t_{\max}}$ has an {\em unique solution} for $0<\delta<1$ and $t_{\max}\geq 1$.
%	
%	{\em Bound the probability of $B^{(2)}_t$}: 
%	Note that $\hat \epsilon_t$ and the samples generated in $\R^{c}_t$ are independent. Thus, we can apply the concentration inequality in Eq.~(\ref{eq:plus}):
%	\begin{align*}
%	&\Pr[\I^{c}_t(\hat S_k) \geq (1 + \hat \epsilon_t)\I(\hat S_k)]
%	\leq \exp\left({-\frac{N_t \I(\hat S_k) {\hat \epsilon_t}^2}{(2+\frac{2}{3}\hat \epsilon_t) n}}\right)  =\frac{\delta}{3 t_{\max}}.
%	\end{align*}
%	The last equation is due to the definition of $\hat \epsilon_t$.	
%	
%	{\em Bound the probability of $B^{(3)}_t$}: Since $\epsilon^*_t$ is fixed and independent from the generated samples, we have
%	\begin{align}
%	\Pr[& \hat \I_t(S^*_k) \leq (1-\epsilon^*_t) \OPT_k]  \leq \exp\left({- \frac{|\R_t| \OPT_k {\epsilon^*_t}^2}{2 n}}\right) \nonumber \\
%	& = \exp\left({-\frac{\Lambda 2^{t-1} \OPT_k \epsilon_0^2 n }{2 n 2^{t-1} \OPT_k}}\right) \\
%	&= 		\exp\left({- \frac{(2+\frac{2}{3}\epsilon_0) \ln (\frac{3 t_{\max}}{\delta})\frac{1}{\epsilon_0^2} 2^{t-1} \OPT_k \epsilon_0^2 n}{ 2(1+\epsilon_0/3)n 2^{t-1} \OPT_k}}\right) \nonumber \\
%	& \leq \exp\left({-\ln \frac{3 t_{\max}}{\delta}}\right) = \frac{\delta}{3 t_{\max}},
%	\end{align}
%	which completes the proof of Lemma.~\ref{lem:bad2}.
%\end{proof}

\begin{Lemma}
	\label{lem:e2e}
	Assume that none of the bad events $B^{(1)}$, $B^{(2)}_t$, $B^{(3)}_t$  ($t =1..t_{\max}$) happen and \ISSA{} stops with some $\epsilon_t \leq \epsilon_0$. We have 
	%\vspace{-0.1in}
	\begin{align}
		&\hat \epsilon_t < \epsilon \text{ and consequently }\\
		&{\hat \I}^{(c)}_t(\hat S_k) \leq (1+\epsilon_0)\I(\hat S_k)
	\end{align}
	%\vspace{-0.25in}
\end{Lemma}
%\begin{proof}
%	Since the bad event $B^{(2)}_t$ does not happen, we have
%	\begin{align}
%	\nonumber \hat \I_t^{(c)}(\hat S_k) \leq (1+\hat \epsilon_t)\I(\hat S_k)
%	\Leftrightarrow \hat \I_t^{(c)}(\hat S_k) \frac{N_t}{n} \leq (1+\hat \epsilon_t)N_t\frac{\I(\hat S_k)}{n}
%	\end{align}
%	
%	When \ISSA{} stops with $\epsilon_t \leq \epsilon_0$, it must satisfy the condition on line 9 of \ISSA{}
%	\[
%		\frac{\I_t^{(c)}(\hat S_k) \cdot |\R^c_t|}{n} \geq \Lambda_1.
%	\]
%	Thus, we have
%	\begin{align}
%	\label{eq:Nt}(1+\hat \epsilon_t)N_t\frac{\I(\hat S_k)}{n} \geq \Lambda_1=1+(1+\epsilon_0)\frac{2+2/3\epsilon_0}{\epsilon_0^2} \ln \frac{3t_{\max}}{\delta}
%	\end{align}
%	From the definition of $\hat \epsilon_t$, it follows that
%	\begin{align}
%	\label{eq:nt}
%	N_t = \frac{2+2/3 \hat \epsilon_t}{\hat\epsilon_t^2} \ln \left(\frac{3t_{\max}}{\delta}\right)\frac{n}{\I(\hat S_k)}
%	\end{align}
%	Substitute the above into (\ref{eq:Nt}) and simplify, we obtain:
%	\begin{align}
%	&(1+\hat \epsilon_t)\frac{2+2/3 \hat \epsilon_t}{\hat\epsilon_t^2} \ln \left(\frac{3t_{\max}}{\delta}\right)\\
%	\geq & (1+\epsilon_0)\frac{2+2/3\epsilon_0}{\epsilon_0^2} \ln \frac{3t_{\max}}{\delta}+1
%	\end{align}
%	Since the function $(1+x)\frac{2+2/3x}{x^2}$ is a decreasing function for $x>0$, it follows that $\hat \epsilon_t < \epsilon_0$.
%\end{proof}

We now obtain the approximation guarantee of \ISSA{}.

%We show that \ISSA{} preserves the $(1-1/e-\epsilon)$-approximation factor of \PIMA{} by the following theorem.
\begin{theorem}
	\label{theo:approx}
	Given a graph $G$, $0 < \delta < 1$, and $0 < \rho < \smash{1-1/e}$, \ISSA{} returns an $\rho$-approximate solution with probability at least $(1-\delta)$.
\end{theorem}
%\begin{proof}
%	Apply union bound for the bad events in Lemmas \ref{lem:cap} and \ref{lem:bad2}. The probability that at least one of the bad events $B^{(1)}, B^{(2)}_t, B^{(3)}_t$  ($t =1..t_{\max}$) happen is at most
%	\begin{align}
%	\delta/3 + \left(\delta/(3t_{\max}) + \delta/(3t_{\max})\right) \times t_{\max} \leq \delta
%	\end{align}
%	
%	In other words, the probability that none of the bad events happen will be at least $1-\delta$. Assume that none of the bad events happen, we shall show that the returned $\hat S_k$ is a $\rho$-approximation solution.
%	
%	
%	If \ISSA{} stops with $|\R_t| \geq N_{\max}$, $\hat S_k$ is a $\rho$-approximation solution, since the bad event $B^{(1)}$ does not happen.
%	
%	Otherwise, \ISSA{} stops at some iteration $t$ and $\epsilon_t \leq \epsilon_0$. We use contradiction method.  
%	Assume that 
%	\begin{align}
%		\label{eq:contrad}\I(\hat S_k) < \rho \OPT_k.
%	\end{align}
%	The proof will continue in the following order
%	\begin{enumerate}[label=(\Alph*)]
%		\item  $\I(\hat S_k) \geq \rho'_t \OPT_k$\\ where $\rho'_t = \sigma(1-\epsilon_t^*)-(\epsilon_1+\hat \epsilon_t+\epsilon_1\hat \epsilon_t)\rho$.
%		\item  $\hat \epsilon_t \leq \epsilon_2$ and  $\epsilon^*_t \leq \epsilon_3$.
%		\item  $\rho_t' \geq \rho_t \geq \rho \Rightarrow \I(\hat S_k) \geq \rho \OPT_k$ (\emph{contradiction}).
%	\end{enumerate}
%	
%	
%	
%	\emph{Proof of (A)}. Since the bad events $B^{(2)}_t$ and $B^{(3)}_t$ do not happen, we have
%	\begin{align}
%		\label{eq:ici} \hat \I_t^{(c)}(\hat S_k) &\leq (1+\hat \epsilon_t)\I(\hat S_k), \text{and}\\
%		\label{eq:iho} \hat \I_t(S^*_k) &\leq (1-\epsilon_t^*) \OPT_k.
%	\end{align}
%	Since $\epsilon_1 \leftarrow \hat \I_t(\hat S_k)/\I^{c}_t(\hat S_k) - 1$, it follows from (\ref{eq:ici}) that
%	\begin{align}
%		\hat \I_t(\hat S_k) =  (1+\epsilon_1)\I^{c}_t(\hat S_k)\leq (1+\epsilon_1)(1 + \hat\epsilon_t) \I(\hat S_k) \nonumber
%	\end{align}	
%	Expand the right hand side and apply (\ref{eq:contrad}), we obtain	
%	\begin{align}
%		\I(\hat S_k) &\geq \hat \I_t(\hat S_k) - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t) \I(\hat S_k) \nonumber \\
%		& \geq \hat \I_t(\hat S_k) - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t) \rho\OPT_k \nonumber
%	\end{align}
%	Since the greedy algorithm in the Max-Coverage guarantees a $\sigma$-approximation, $\hat \I_t(\hat S_k) \geq \sigma \hat \I_t(S^*_k)$. Thus
%	\begin{align}		
%		&\I(\hat S_k)  \geq \sigma \hat \I_t(S^*_k)  - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t)\rho \OPT_k \nonumber \\
%		&\geq \sigma(1-\epsilon^*_t) \OPT_k  - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t)\rho \OPT_k  \nonumber \\
%		&\geq \rho'_t \OPT_k, \nonumber
%	\end{align}
%	where $\rho'_t = \sigma (1 - \epsilon^*_t) - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t)\rho$.
%	
%	\emph{Proof of (B)}. We show that $\hat \epsilon_t \leq \epsilon_2$. Since, $\epsilon_2 = \epsilon_0 \sqrt{\frac{n(1+\epsilon_0)}{2^{t-1} \I^{c}_t (\hat S_k)}}$, we have
%	\[
%		\frac{1}{\epsilon_0^2} = \frac{1}{\epsilon_2^2} \frac{n}{2^{t-1}} \frac{1+\epsilon_0}{\I^{c}_t(\hat S_k)}.
%	\]
%	Expand the number of \ROS{} samples in iteration $t$, $N_t = 2^{t-1} \Lambda$, and apply the above equality, we have 
%	\begin{align}
%		N_t &=  2^{t-1} (2+2/3\epsilon_0)\frac{1}{\epsilon_0^2} \ln \frac{3t_{\max}}{\delta} \\
%		&=  2^{t-1} (2+2/3\epsilon_0)\frac{1}{\epsilon_2^2}  \frac{n}{2^{t-1}} \frac{1+\epsilon_0}{\I^{c}_t(\hat S_k)}  \ln \frac{3t_{\max}}{\delta} \\
%		&= (2+2/3\epsilon_0)\frac{1}{\epsilon_2^2} \frac{(1+\epsilon_0)n}{\I^{c}_t(\hat S_k)}  \ln \frac{3t_{\max}}{\delta}
%	\end{align}
%	On the other hand, according to Eq.~(\ref{eq:nt}), we also have,
%	\begin{align}
%		N_t = \frac{2+2/3 \hat \epsilon_t}{\hat\epsilon_t^2} \ln \left(\frac{3t_{\max}}{\delta}\right)\frac{n}{\I(\hat S_k)}.
%	\end{align}
%	Thus
%	\begin{align*}
%		& (2+2/3\epsilon)\frac{1}{\epsilon_2^2} \frac{1+\epsilon_0}{\I^{c}_t(\hat S_k)} = \frac{2+2/3 \hat \epsilon_t}{\hat\epsilon_t^2} \frac{1}{\I(\hat S_k)}\\
%		\Rightarrow &\frac{\hat \epsilon_t^2}{\epsilon_2^2} = \frac{2+2/3 \hat \epsilon_t}{2+2/3 \epsilon_0}  \frac{\I^{c}_t(\hat S_k)}{(1+\epsilon_0)\I(\hat S_k)} \leq 1
%	\end{align*}
%	The last step is due to Lemma \ref{lem:e2e}, i.e., $\I^c_t(\hat S_k) \leq (1+\epsilon_0)\I(\hat S_k)$ and $\hat \epsilon_t \leq \epsilon_0$. Therefore, $\hat\epsilon_t \leq \epsilon_2$.
%	
%	We show that $\epsilon^*_t \leq \epsilon_3$. According to the definition of $\epsilon^*_t$ and $\epsilon_3$, we have
%	\begin{align*}
%		\frac{(\epsilon^*_t)^2}{\epsilon_3^2} &=\frac{n}{(1+\epsilon/3)2^{t-1} \OPT_k} / 
%		\frac{n(1+\epsilon_0)\rho}{(1+\epsilon_0/3)2^{t-1} \I^{c}_t (\hat S_k)}\\
%		=& \frac{\I^{c}_t (\hat S_k)}{\OPT_k (1+\epsilon_0)\rho}
%		\leq \frac{\I_t (\hat S_k)}{\OPT_k \rho}\leq 1
%	\end{align*}
%	The last two steps follow from Lem.~\ref{lem:e2e}, $\I^c_t(\hat S_k) \leq (1+\epsilon_0)\I(\hat S_k)$ and the assumption (\ref{eq:contrad}), respectively. Thus, $\epsilon_t^* \leq \epsilon_3$.
%	
%	\emph{Proof of (C)}. Since $1+\epsilon_1 = \hat \I_t(\hat S_k)/\I^{c}_t(\hat S_k) \geq 0$ and $\epsilon_2 \geq \hat \epsilon_t >0$ and 
%	$\epsilon_3 \geq \epsilon^*_t >0$, we have
%	\begin{align}
%		\rho_t' &= \sigma (1-\epsilon^*_t) - (\epsilon_1 + \hat\epsilon_t + \epsilon_1 \hat\epsilon_t)\rho \\
%		&= \sigma (1-\epsilon^*_t) - (\epsilon_1 + \hat\epsilon_t (1+\epsilon_1))\rho \\
%		& \geq \sigma (1-\epsilon_3 ) - (\epsilon_1 + \epsilon_2 (1+\epsilon_1))\rho \\
%		&= \rho_t \geq \rho.
%	\end{align}
%	
%	This completes the proof.
%\end{proof}


%\textbf{Optimal Sampling.}
%Similar to \ISSA{}, the type-2 optimality in terms of \ROS{} samples generated is achieved in \ISSA{} under the condition that $\rho < 1-1/e$.
%
%\begin{theorem}
%	\label{theo:odima}
%	Given a graph $G$, $\underline{ \smash{0 \leq \rho < 1-1/e}}$ and $0\leq \delta \leq 1$, let $N^2_{min}(\epsilon,\delta)$ be the type-2 minimum threshold of \ROS{} samples to guarantee the $\rho$-approximate solution. \ISSA{} generates at most, to within a constant factor, $N^2_{min}(\epsilon,\delta)$ \ROS{} samples with the probability of at least $(1-2\delta)$.
%\end{theorem}
%
%The proof follows directly from that of \ISSA{} with a note that the runtime approximation bound provided by the \textsf{Greedy} algorithm is at least $1-1/e$, thus, \ISSA{} always stops earlier than \ISSA{} under the same sample set. In addition, \ROS{} and \RIS{} are viewed as having the same roles.

\subsection{Anytime Approx. Algorithm | Beyond $(1-1/e)$} 
In many cases of the input graph $\G$, $k$, \ISSA{} can provide a better approximation guarantee $\rho \geq 1-1/e$ due to the runtime approximation bound. This happens when the first stopping condition $\rho_t \geq \rho$ is met. Conversely, in other cases of $\rho \geq 1-1/e$ and within $N_{\\max}$ \ROS{} samples, \ISSA{} cannot provide the guarantee, the second stopping condition takes effect as a guarding terminator. In those cases, the returned solution $\hat S_k$ is at least $\max\{(1-1/e-|\epsilon|), \rho_t \}$-optimal. 
%As such, the type-2 optimal sampling requirement only holds when $\rho < 1 - 1/e$.

Moreover, due to the dynamic guarantee $\rho_t$ at every iteration, \ISSA{} provides an \textit{anytime} approximation guarantee. \ISSA{} can be stopped at anytime (any iteration $t$) in the middle and return the current candidate solution $\hat S_k$ with the provided guarantee of $\rho_t$. In another way, we can set the time limit for \ISSA{} to run and it will return the best-effort solution $\hat S_k$ with a approximation guarantee of $\rho_t$ when the time limit has been used up at iteration $t$.
